A (Weakly) Polynomial Algorithm for AIVF Coding

It is possible to improve upon Tunstall coding using a collection of multiple parse trees. The best such results so far are Iwata and Yamamoto's maximum cost AIVF codes. The most efficient algorithm for designing such codes is an iterative one that could run in exponential time. In this paper, we show that this problem fits into the framework of a newly developed technique that uses linear programming with the Ellipsoid method to solve the minimum cost Markov chain problem. This permits constructing maximum cost AIVF codes in (weakly) polynomial time.

==> DP.tex <==


\begin{algorithm} 
\caption{Fills in the $\OPT(i:d)$ table and constructs the $t^{(i)}_d$ satisfying $\Cost\left(t^{(d)}_i\right)=\OPT(i:d)$ }\label{alg:dp}
\begin{algorithmic}[1]
\Require $D \geq 2$,  $\{\alpha_i|i \in \mathcal{I}_{|S|-1}\}$ and $\{x_j|1\leq j \leq m-1\}$.
\textbf{Ensure:} $t_i^{(D)}$ and $\OPT(i:D)$ satisfy $t_i^{(D)}:=\argmax\limits_{s_i^{(D)} \in \mathcal{T}_{i}^{(D)}} \Cost\left(s^{(D)}_i\right)$ and $\OPT(i:D)=\Cost\left(t^{(D)}_i\right)$ respectively for $i\in \mathcal{I}_{|S|-1}$.
\algrenewcommand\algorithmicrequire{\textbf{Initialization:}}
\Require $t_i^{(1)} \gets $Root and $\OPT(i:1) \gets 0 $ for $ i\in{I}_{|S|-1}\ $.
\For{$d=2$ to $D$ }
\For{$i=0$ to $|S|-3$ }
\State  $\OPT(i:d) \gets  \max\limits_{1 \le l < d-1}
            \Bigl( \alpha_i + \alpha_i \cdot \OPT(0:l)+(1- \alpha_i) \cdot \OPT(i+1:d-l) \Bigr)$ \label{line:opt update}
\State  \hspace*{0.56in}$l' \gets  \argmax\limits_{1 \le l < d-1}
            \Bigl( \alpha_i + \alpha_i \cdot \OPT(0:l)+(1- \alpha_i) \cdot \OPT(i+1:d-l) \Bigr)$         \label{line:maximum l}
\State   $t^{(d)}_i \gets \Tie_i\left( t^{(l')}_0, t^{(d-l')}_{i+1} \right)$ \label{line:t_i update}           
\EndFor
\State  $\OPT(|S|-2:d) \gets  \max\limits_{1 \le l < d-1}
            \Bigl( 1 + \alpha_{|S|-2} \cdot \OPT(0:l)+(1- \alpha_{|S|-2}) \cdot \OPT(0:d-l) \Bigr)$
\State  \hspace*{0.93in}$l' \gets  \argmax\limits_{1 \le l < d-1}
            \Bigl( 1 + \alpha_{|S|-2} \cdot \OPT(0:l)+(1- \alpha_{|S|-2}) \cdot \OPT(0:d-l) \Bigr)$     
\State   $t^{(d)}_{|S|-2} \gets \Tie_i\left( t^{(l')}_0, t^{(d-l')}_{0} \right)$           \label{line:second t_i update} 
\EndFor \\
\Return $\left\{\OPT(i:D), t^{(D)}_i \mid i \in\mathcal{I}_{|S|-1}\right\}$
\end{algorithmic}
\end{algorithm}

\begin{figure}[ht]
\begin{minipage}{0.45\textwidth}
\begin{center}
\begin{tikzpicture}[
  node/.style={circle,draw,minimum width=0mm,inner sep=0, fill=black},
  non-codeword/.style={circle,draw,minimum width=1mm,inner sep=0},
  subtree1/.style={isosceles triangle,draw,shape border rotate=90,isosceles triangle stretches=true, minimum height=12mm,minimum width=12mm,inner sep=0,yshift={-1.5mm},line width=0.8pt},
  subtree2/.style={draw,shape border uses incircle,
  isosceles triangle,isosceles triangle apex angle=90,
  shape border rotate=-135,yshift=0.5mm,xshift=-9mm,minimum height=12mm,minimum width=12mm,line width=0.8pt},
  level 1/.style={sibling distance=30mm},
]
  \node[node] {}
    [child anchor=north]
    child {node[subtree1]{$s_0^{(l)}$} edge from parent node[left,draw=none,yshift=1.5mm,xshift=2mm]{$a_i$}} 
    child {node[subtree2] {$s_{i+1}^{(r)}$}};
\end{tikzpicture}
\end{center}
\caption*{$\Tie_{i}\Bigl(s_0^{(l)},s_{i+1}^{(r)}\Bigr)$}
\end{minipage}
\hspace{10pt} 
\begin{minipage}{0.45\textwidth}
\begin{center}
\begin{tikzpicture}[
  node/.style={circle,draw,minimum width=0mm,inner sep=0, fill=black},
  non-codeword/.style={circle,draw,minimum width=1mm,inner sep=0},
  subtree1/.style={isosceles triangle,draw,shape border rotate=90,isosceles triangle stretches=true, minimum height=12mm,minimum width=12mm,inner sep=0,yshift={-1.5mm},line width=0.8pt},
  level 1/.style={sibling distance=15mm},
]
  \node[node] {}
    [child anchor=north]
    child {node[subtree1]{$s_0^{(l)}$} edge from parent node[left,draw=none,yshift=1.5mm,xshift=0mm]{$a_{|S|-2}$}} 
    child {node[subtree1] {$s_{0}^{(r)}$}edge from parent node[right,draw=none,yshift=1.5mm,xshift=0mm]{$a_{|S|-1}$}};
\end{tikzpicture}
%\captionof{figure}{A caption.}
\end{center}
\caption*{$\Tie_{|S|-2}\Bigl(s_0^{(l)},s_{0}^{(r)}\Bigr)$}
\end{minipage}
\caption{On the left-hand we can see an Illustration of how the trees in $\mathcal{T}_i$ can be decomposed for $i\in\mathcal{I}_{|S|-2}$ and on the right-hand side we can see how a the trees in $\mathcal{T}_{|S|-2}$ can be decomposed.}
\label{fig:tree dissection}
\end{figure}

%At each iteration of our algorithm we are required to solve a local optimization problem that involves finding in order to find the highest hyperplane of each type at that point.Lets say that $\mathcal{T}_{i}$ denotes the set of trees $t_i$ satisfying (p1)-(p3), and $\mathcal{T}_{i}^{(D)}$ is the set of trees that are in $\mathcal{T}_{i}$ that have exactly $D$ codewords. This means that for a fixed set $\{x_j|1\leq j \leq n-1\}$ we want to find the tree $t_0 \in \mathcal{T}_{0}^{(D)}$ that maximizes $E[L_{t_0}(S)] + \sum_{j=1}^{m-1}q_j(t_0)\cdot x_j$ and the tree $t_i \in \mathcal{T}_{i}^{(D)}$ that maximizes $E[L_{t_i}(S)] + \sum_{j=1}^{m-1}q_j(t_i)\cdot x_j-x_i$ for every $i>0$.\\ Since the $x_i$s are fixed this is equivalent to finding the tree $t_i \in \mathcal{T}_{i}^{(D)}$ that maximizes 

Lets say that $\mathcal{T}_{i}$ denotes the set of trees $t_i$ satisfying (p1)-(p3), and $\mathcal{T}_{i}^{(D)}$ is the set of trees that are in $\mathcal{T}_{i}$ that have exactly $D$ codewords. Consider the fixed set$\{x_j|1\leq j \leq m-1\}$. We define 
\begin{equation}
    \Cost\left(t_i\right)=E[L_{t_i}(S)] + \sum_{j=1}^{m-1}q_j(t_i)\cdot x_j
\end{equation}
for $t_i\in\mathcal{T}_{i}$.
%Consider the fixed set$\{x_j|1\leq j \leq n-1\}$. 
\\In order to find optimal AIVF codes we are required to solve a local optimization problem that involves finding the tree $t_0 \in \mathcal{T}_{0}^{(D)}$ that maximizes $E[L_{t_0}(S)] + \sum_{j=1}^{m-1}q_j(t_0)\cdot x_j$ and the tree $t_i \in \mathcal{T}_{i}^{(D)}$ that maximizes $E[L_{t_i}(S)] + \sum_{j=1}^{m-1}q_j(t_i)\cdot x_j-x_i$ for every $i>0$. Since the $x_i$s are fixed this is equivalent to finding the tree $t_i \in \mathcal{T}_{i}^{(D)}$ that maximizes $\Cost\left(t_i\right)$ for each $i\in\mathcal{I}_{|S|-1}$. We now look at a couple of simple observations that will help us develop a straight forward approach to find these trees.

For $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$, $s_{i+1}^{(r)} \in \mathcal{T}_{i+1}^{(r)}$ and $i\in\mathcal{I}_{|S|-2}$ we define $\Tie_{i}\Bigl(s_0^{(l)},s_{i+1}^{(r)}\Bigr)$ to be the unique tree in $\mathcal{T}_{i}$ that is created by taking $s_{i+1}^{(r)}$ and adding a new edge labeled $a_i$ to its root that connects to $s_0^{(l)}$. Consequently this new tree has $l+r$ codewords and is therefor in $\mathcal{T}_{i}^{(l+r)}$. Note that the converse is true, that is for any $s_{i}^{(D)}\in\mathcal{T}_{i}^{(D)}$ satisfying $D\geq2$ and $i\in\mathcal{I}_{|S|-2}$ there exists $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{i+1}^{(r)} \in \mathcal{T}_{i+1}^{(r)}$ such that $l,r\geq1$, $l+r=D$ and $s_{i}^{(D)}:=\Tie_{i}\Bigl(s_0^{(l)},s_{i+1}^{(r)}\Bigr)$. We can see an illustration of this on the Left hand side of figure \ref{fig:tree dissection}.

For $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{0}^{(r)} \in \mathcal{T}_{0}^{(r)}$ we define $\Tie_{|S|-2}\Bigl(s_0^{(l)},s_{0}^{(r)}\Bigr)$ to be the unique tree in $\mathcal{T}_{|S|-2}$ that is created by taking a new node as the root having 2 edges labeled $a_{|S|-2}$ and $a_{|S|-1}$ connecting to $s_{0}^{(l)}$ and $s_0^{(r)}$ respectively. Consequently this new tree has $l+r$ codewords and is therefor in $\mathcal{T}_{|S|-2}^{(l+r)}$. Note that similar to the previous case, the converse is true, that is for any $s_{|S|-2}^{(D)}\in\mathcal{T}_{|S|-2}^{(D)}$ satisfying $D\geq2$ there exists $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{0}^{(r)} \in \mathcal{T}_{0}^{(r)}$ such that $l,r\geq1$, $l+r=D$ and $s_{|S|-2}^{(D)}:=\Tie_{|S|-2}\Bigl(s_0^{(l)},s_{0}^{(r)}\Bigr)$. We can see an illustration of this on the right hand side of figure \ref{fig:tree dissection}.

Now Consider $s_{i}^{(D)}\in\mathcal{T}_{i}^{(D)}$ satisfying $D\geq2$ and $i\in\mathcal{I}_{|S|-2}$ and consider the unique trees $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{i+1}^{(r)} \in \mathcal{T}_{i+1}^{(r)}$ satisfying $s_{i}^{(D)}:=\Tie_{i}\Bigl(s_0^{(l)},s_{i+1}^{(r)}\Bigr)$. let's say we're about to encode an input string using $s_{i}^{(D)}$. The probability that the first character of our input is $a_i$ is equal to $\frac{p(a_i)}{\sum_{j=i}^{m-1}p(a_j)}$. Denote $\alpha_{i}=\frac{p(a_i)}{\sum_{j=i}^{m-1}p(a_j)}$. This means that the probability that we will parse our next codeword using $s_{0}^{(l)}$ and $s_{i+1}^{(r)}$ is $\alpha_i$ and $1-\alpha_i$ respectively. Using this observation we can say:
\begin{equation}
    \forall{j\in\mathcal{I}_{|S|-1}}:\space q_j\Bigl(s_i^{(D)}\Bigr)=\alpha_i 
 \cdot q_j\Bigl(s_0^{(l)}\Bigr)+(1-\alpha_i) \cdot q_j\Bigl(s_{i+1}^{(r)}\Bigr)
\end{equation}
\begin{equation}
    E[L_{s_{i}^{(D)}}(S)]=\alpha_i \cdot \Bigl(E[L_{s_0^{(l)}}(S)]+1\Bigr)+(1-\alpha_i) \cdot E[L_{s_{i+1}^{(r)}}(S)]
\end{equation}
Hence
\begin{eqnarray} \label{eq:type i cost decomposition} \nonumber
\Cost\Bigl(s_i^{(D)}\Bigr)&=&E[L_{s_i^{(D)}}(S)]+ \sum_{j=1}^{m-1}q_j\Bigl(s_i^{(D)}\Bigr)\cdot x_j\\ \nonumber
&=&\alpha_i \cdot \Bigl(E[L_{s_0^{(l)}}(S)]+1\Bigr)+(1-\alpha_i) \cdot E[L_{s_{i+1}^{(r)}}(S)]+\sum_{j=1}^{m-1}\Biggl(\alpha_i \cdot q_j\Bigl(s_0^{(l)}\Bigr)+(1-\alpha_i) \cdot q_j\Bigl(s_{i+1}^{(r)}\Bigr)\Biggr)\cdot x_j\\ \nonumber
&=&\alpha_i+\alpha_{i} \cdot \Biggl(E[L_{s_0^{(l)}}(S)]+\sum_{j=1}^{m-1}q_j\Bigl(s_0^{(l)}\Bigr)\cdot x_j\Biggr)+(1-\alpha_i) \cdot \Biggl(E[L_{s_{i+1}^{(r)}}(S)]+q_j\Bigl(s_{i+1}^{(r)}\Bigr)\cdot x_j\Biggr)\\ 
&=&\alpha_i+\alpha_{i}\cdot \Cost\Bigl(s_0^{(l)}\Bigr)+(1-\alpha_i)\cdot \Cost\Bigl(s_{i+1}^{(r)}\Bigr) 
\end{eqnarray}
Now Consider $s_{|S|-2}^{(D)}\in\mathcal{T}_{|S|-2}^{(D)}$ satisfying $D\geq2$ and consider the unique trees $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{0}^{(r)} \in \mathcal{T}_{0}^{(r)}$ satisfying $s_{|S|-2}^{(D)}:=\Tie_{|S|-2}\Bigl(s_0^{(l)},s_{0}^{(r)}\Bigr)$. Denote $\alpha_{|S|-2}=\frac{p(a_{|S|-2})}{p(a_{|S|-2})+p(a_{|S|-1})}$. Similar to before, we can say:
\begin{eqnarray}
    \nonumber
    \Cost\Bigl(s_{|S|-2}^{(D)}\Bigr)&=&E[L_{s_{|S|-2}^{(D)}}(S)]+ \sum_{j=1}^{m-1}q_j\Bigl(s_{|S|-2}^{(D)}\Bigr)\cdot x_j\\ \nonumber
    &=&\alpha_i \cdot \Bigl(E[L_{s_0^{(l)}}(S)]+1\Bigr)+(1-\alpha_i) \cdot \Bigl(E[L_{s_{0}^{(r)}}(S)]+1\Bigr)+\sum_{j=1}^{m-1}\Biggl(\alpha_i q_j\Bigl(s_0^{(l)}\Bigr)+(1-\alpha_i) \cdot q_j\Bigl(s_{0}^{(r)}\Bigr)\Biggr)\cdot x_j\\
    &=&1+\alpha_{|S|-2}\cdot \Cost\Bigl(s_0^{(l)}\Bigr)+(1-\alpha_{|S|-2})\cdot \Cost\Bigl(s_{0}^{(r)}\Bigr)
\end{eqnarray}
These observations give way for a divide and conquer approach that will help us use dynamic programming to solve this problem.


Algorithm \ref{alg:dp} is the same algorithm proposed by Iwata and Yamamoto in ~\cite{AIVF-iterative} which is an extension of the algorithm proposed by Dubé and Haddad ~\cite{dube-haddad} and has been rewritten using our change of variables.\\
\begin{theorem} \label{theorem:Tunstal DP}
The output $\left\{\OPT(i:D), t^{(D)}_i \mid i \in\mathcal{I}_{|S|-1}\right\}$ of Algorithm \ref{alg:dp} satisfies $t_i^{(D)}=$ $\argmax\limits_{s_{i}\in \mathcal{T}_{i}^{(D)}} \Cost(s_i)$ and $\OPT(i:D)=\Cost\Bigl(t_i^{(D)}\Bigr)$ for $i\in\mathcal{I}_{|S|-1}$.
\end{theorem}

\begin{proof}
By induction on that $d$ we show that $t_{i}^{(d)}$ and $\OPT(i:d)$ derived from Algorithm \ref{alg:dp} satisfy $t_i^{(d)}:=$ $\argmax\limits_{t_{i}\in \mathcal{T}_{i}^{(d)}} \Cost(t_i)$ and $\OPT(i:d)=\Cost\Bigl(t_i^{(d)}\Bigr)$ for $i\in\mathcal{I}_{|S|-1}$.\\
For the base case we have $t_i^{(1)}:=$Root and $\OPT(i:1)=0$ for $i\in\mathcal{I}_{|S|-1}$ where Root is a tree with only one node. For the inductive step, consider the statement true for all the values less than $d$ and consider the tree $s_{i}^{(d)} \in \mathcal{T}_{i}^{(d)}$ where $i\in\mathcal{I}_{|S|-2}$ and $s_i^{(d)}=$ $\argmax\limits_{s_{i}\in \mathcal{T}_{i}^{(d)}} \Cost(s_{i})$.\\ 
As mentioned before, we know there exists unique trees $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{i+1}^{(d-l)} \in \mathcal{T}_{i+1}^{(d-l)}$ such that $1 \leq l \leq d-1$ and $s_{i}^{(d)}:=\Tie_{i}\Bigl(s_0^{(l)},s_{i+1}^{(d-l)}\Bigr)$. Now considering equation \ref{eq:type i cost decomposition}, in order for $s_{i}^{(d)}$ to maximize $\Cost\Bigl(s_{i}^{(d)}\Bigr)$, $s_{0}^{(l)} \in \mathcal{T}_{0}^{(l)}$ and $s_{i+1}^{(d-l)} \in \mathcal{T}_{i+1}^{(d-l)}$ must maximize $\Cost\Bigl(s_{0}^{(l)}\Bigr)$ and $\Cost\Bigl(s_{i+1}^{(d-l)}\Bigr)$ respectively. In other words $s_{0}^{(l)}:=t_{0}^{(l)}$ and $s_{i+1}^{(d-l)}:=t_{i+1}^{(d-l)}$. This means that in order to find $s_i^{(d)}$ we can go through all possibilities of $l$ and see in which case $\Cost\Bigl(s_i^{(d)}\Bigr)$ is maximized, Which is what's happening in line \ref{line:maximum l} and \ref{line:t_i update} of algorithm \ref{alg:dp}. We can also see that in line \ref{line:opt update}, $\OPT(i:d)$ is being calculated accordingly.
In a similar fashion we can show that the tree  $s_{|S|-2}^{(d)}$ satisfying $s_{|S|-2}^{(d)}:=\argmax\limits_{s_{|S|-2}\in \mathcal{T}_{|S|-2}^{(d)}} \Cost(s_{|S|-2})$ can be found by going through all possibilities of $l$ satisfying $1\leq l\leq d-1$ and observing for which value it maximizes $\Cost\Biggl(\Tie_{|S|-2}\Bigl(t_0^{(l)},t_{0}^{(d-l)}\Bigr)\Biggr)$ and calculating $\OPT(|S|-2:d)$ accordingly. This completes our inductive step and therefore proves the theorem.
\end{proof}
\textbf{Time complexity:} The algorithm that we propose for finding optimal AIVF Code trees is an iterative one that uses this dynamic programming procedure at each iteration, however as we'll see later, other than the last procedure, we don't make use of the trees themselves but rather only their costs, this means that we can use 2 versions of the dynamic programming, one of which only computes the costs of the trees, and the other constructs the trees as well. Since the latter is only used once, this means that we can use a much simpler algorithm for the rest of the iterations. We will now analyze these two versions.
\begin{proposition}
    Algorithm \ref{alg:dp} can be modified to find the costs of the final trees in $O(D^2\cdot m)$ running time.
\end{proposition}
\begin{proof}
    Our modification is simple, by omitting lines \ref{line:t_i update} and \ref{line:second t_i update} our dynamic programming will only fill in the $OPT$ tale which gives us the desired final costs. It is easy to see that we have three loops, having sizes of at most $D$,$m$ and $D$ respectively, therefor the running time is $O(D^2\cdot m)$.
\end{proof}
Before we calculate the time complexity of finding the final trees we will prove a bound on the size of the the trees.
\begin{lemma}
    The maximum size of any type AIVF Code tree with $D$ code words is $2D$.
\end{lemma}
\begin{proof}
    We know that each node either has a codeword assigned to it or it's a complete node. Since there are $D$ elements in our dictionary then there are exactly $D$ nodes with codewords assigned to them. If our tree had more than $2D$ nodes then it would have more than $D$ complete nodes, This would mean that our tree has at least $D$ nodes having degree of at least 2, and it is easy to see that such tree would have at least $D+1$ leafs, resulting in more than $D$ codewords which gives us a contradiction.
\end{proof}
\begin{proposition}
    Algorithm \ref{alg:dp} can find the final trees in $O(D^2\cdot m)$ running time.
\end{proposition}
\begin{proof}
    Consider the following modification; We run through algorithm \ref{alg:dp} but instead of doing the Tie operations at line \ref{line:t_i update} and \ref{line:second t_i update} we just save the corresponding value of $l^{\prime}$ for each $d$ and $i$ in a separate table. The reason we do this is because we don't actually need to create every tree and we can just use this new table to recursively build the final trees after the loops are over. This doesn't change the time complexity but it does decrease the space complexity.\\
    Call this new table $E$. This means that $E(i:d)$ tells us how many codewords are in the left subtree of $t_{i}^{(d)}$ when decomposed according to figure \ref{fig:tree dissection}. Using this information we can recursively create the left and right subtrees in order to find $t_{i}^{(d)}$. Creating the final trees with this procedure has time complexity of $O(m\cdot D)$ because at each step we are adding at least one edge and then recursively finding the left and right subtrees. Since each step takes $O(1)$ time and our trees have at most $2D$ nodes, we create each tree in $O(D)$ time and find all the final trees in $O(mD)$ which doesn't affect the time of filling in the tables resulting in an $O(D^2\cdot m)$ overall run time.
\end{proof}
\textbf{Generalized Dynamic Programming:} \newline
Consider $P\subseteq \mathcal{I}_{m-1}$ such that $0\in P$ and Consider the problem of adding the constraint $q_j(t_{i}^{(d)})=0$ for every $j\notin P$ and $i\in \mathcal{I}_{m-1}$. This means we want to find the trees having the optimal costs defined previously, with the added constraint that each tree has a transition probability of zero for trees having having a type that is not in $P$. The reason that we consider such case will become clear later in the paper.\\
Modifying the dynamic programming in this case is simple. Using the decomposition in figure \ref{fig:tree dissection}, we can see that in order for $s_{i}^{(d)}$ to have the optimal cost between trees that have the added constraint, its subtrees need to be optimal trees that satisfy the added constraint, which means that we can use the exact same dynamic programming, the only difference is that the initialization is going to be different.Consider $j\in \mathcal{I}_{m-2}$ and let $i\in \mathcal{I}_{m-2}$ be the smallest number satisfying $j < i$ and $i \in P$, if no such $i$ exists then let $i=m$. We can see that in this case there are no type $j$ trees having less than $i-j$ codewords and there is exactly one type $j$ tree having $i-j$ codewords which is created by taking a root node having $i-j$ edges with $a_j,a_{j+1},..., a_{i-1}$ as their labels. Using this fact we can initialize the dynamic programming by first adding this information into the table. The rest of the dynamic programming will be exactly the same, we just have to take care in the fact some trees might not be possible.


==> TunstallCoding.tex <==
\textbf{Introduction.} 
Consider a stationary memoryless source with alphabet $S=\{a_0,a_1,...,a_{m-1}\}$ such that the symbol $a_i$ is generated with probability $p(a_i)$ for each $i\in \mathcal{I}_{|S|}$, where $\mathcal{I}_{n}$ denotes the integer set $\{0,1,..,n-1\} $. Without loss of generality we assume that $p(a_0)\geq p(a_1)\geq ... \geq p(a_{m-1})$. Tunstall Code ~\cite{tunstall-original} uses a dictionary $\mathcal{D}$ of variable-length prefix-free phrases of the source symbols and maps each one of them to a codeword of fixed-length.\\
Tunstall Coding is usually considered optimal amongst variable-to-fixed (VF) codes in the sense that it achieves the smallest coding rate $R(\mathcal{D},s):=\frac{log D}{E[L(S)]}$, where $E[L(S)]$ is the average length of the phrases parsed by dictionary $\mathcal{D}$ and $D=|\mathcal{D}|$. But to be more accurate, Tunstall Coding is only optimal when considering prefix-free dictionaries. However, it is not necessary for VF codes to have prefix-free Dictionaries. The dictionary only needs to be exhaustive. Yamamoto and Yokoo ~\cite{aivf-original} proposed the AIFV (almost instantaneous VF) code which was later extended by Dubé and Haddad ~\cite{dube-haddad}. This generalization of tunstall coding uses multiple dictionaries that aren't necessarily prefix-free and as a result, it achieves a better coding rate than Tunstall Coding.
\newline
We now define these two methods in more detail and give examples of how they work. In order to keep things simple we mostly use the same notations and definitions used in ~\cite{AIVF-iterative}.
%\newline\newline
%\textbf{Notations, Definitions and Conventions.} 
%Without loss of generality we assume that $p(a_0)\geq p(a_1)\geq ... p(a_{m-1})$. Let $D=|\mathcal{D}|$.
\newline\newline A. Tunstall Coding \newline
%\tikzset{node distance = 5mm and 10mm}
\begin{figure}[ht] 
    \centering
    \subfloat[Parse Tree]{
\begin{tikzpicture}[
node/.style={circle,draw,minimum width=6.3mm,inner sep=0}, level 1/.style={sibling distance=15mm},level distance=12mm, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)},baseline
]
]
\node [node]{\tiny $1.0$}
[child anchor=north]
child {node[node]{\tiny $0.6$}
child {node[node]{\tiny $0.36$} 
child {node[node]{\tiny $0.216$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
child {node[node]{\tiny $0.108$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}}
child {node[node]{\tiny $0.036$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
child {node[node]{\tiny $0.18$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}}
child {node[node]{\tiny $0.06$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}
}
  child {node[node]{\tiny $0.3$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}}
  child {node[node]{\tiny $0.1$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}};
\end{tikzpicture}}
\hspace{30pt}
%\hfill
%\renewcommand{\arraystretch}{1.3}
\subfloat[Dictionary Table]{
\begin{tabular}[t]{c|c|c}
$\ell$ & $w_{ \ell \in\mathcal{D}}$  & $P_{C}(w_{ \ell})$                     \\ \hline
1 & $a_0 a_0 a_0$ & 0.216 \\ \hline
2 & $a_0 a_0 a_1$ & 0.108                     \\ \hline
3 & $a_0 a_0 a_2$ & 0.036                     \\ \hline
4 & $a_0 a_1$  & 0.18                      \\ \hline
5 & $a_0 a_2$  & 0.06                      \\ \hline
6 & $a_1$   & 0.3                       \\ \hline
7 & $a_2$   & 0.1                      
\end{tabular}}
\caption{The parse tree and dictionary $\mathcal{D}$ of Tunstall code for the source of $S=\{a_0,a_1,a_2\}$ and $p(a_0)=0.6$, $p(a_1)=0.3$, $p(a_2)=0.1$ and $D=7$.}
\label{fig:tunstall example}
\end{figure}

\begin{algorithm}
\caption{Tunstall algorithm to design dictionary of Tunstall code}\label{alg:tun}
\begin{algorithmic}[1]
\Require $k\in\mathbb{Z}^{+}$ and $\{p(a_i)$ $|$ $i\in \mathcal{I}_{|S|}\}$.
\Ensure $\mathcal{D}$ such that $D=|S|+(|S|-1)k$.
\algrenewcommand\algorithmicrequire{\textbf{Initialization:}}
\Require $t \gets $Root +$S$. \Comment{Root denotes a tree consisting of only one node}
\For{$i=1$ to $k$ do}
\State $w_{max} \gets $ $\argmax\limits_{w\in\mathcal{D}(t)} p_{C}(w)$ \Comment{$\mathcal{D}(t)$ is the dictionary induced by parse tree t.}
\State $t \gets t+\{w_{max} \cdot a_i $ $|$ $i\in \mathcal{I}_{|S|}\}$
\EndFor \\
\Return $\mathcal{D}(t)$
\end{algorithmic}
\end{algorithm}
Figure \ref{fig:tunstall example} shows an example of a parse tree and dictionary of a Tunstall code. Every internal node has $|S|$ children each corresponding to a different source symbol and a different codeword is assigned to each leaf. The parse dictionary $\mathcal{D}=\{w_\ell|\ell=1,2,...,D\}$ consists of the source symbol strings from the root to all the leaves, and $D=|S|+(|S|-1)k$ for some $k\geq0$.
\newline
In order to encode the source sequence using dictionary $\mathcal{D}$ we first map a prefix $w_\ell \in \mathcal{D}$ of the source sequence to the corresponding code word $\ell$ of fixed-length and then remove the prefix $w_\ell$ from the source sequence. We continue this encoding process until the source sequence becomes empty and we ignore the case where a few symbols might be left that cannot be parsed by the dictionary.
\newline
Since we consider that the symbols of the source sequence are generated independently we know that the probability $p_{W}(w)$ of phrase $w\in S^{+}$ can be calculated by 
\begin{equation} \label{eq:pw}
    p_{W}(w)=\prod_{i=1}^{n}p(c_i)
\end{equation} where $w=c_1c_2...c_n$ is the character decomposition of w and $p(\lambda)=1$ where $\lambda$ is the empty string. In Figure \ref{fig:tunstall example} we can see that the values of each node is the probability $p_{W}(w)$ of the phrase w given by the path from the root to that node. In the case of Tunstall codes the occurrence probability $p_C(w_\ell)$ of a parse phrase $w_\ell \in \mathcal{D}$ is given by
\begin{equation} \label{to:tunstall occurrence}
    p_C(w_\ell)=p_{W}(w_\ell).
\end{equation}
We can now easily see that the average parse length $E[L_{TUNSTALL}(S)]$ of Tunstall code with dictionary $\mathcal{D}$ for source S can be calculted by \ref{tunstall average}
\begin{equation}\label{tunstall average}
    E[L_{TUNSTALL}(S)]:=\sum_{w_\ell \in \mathcal{D}}p_C(w_\ell)l(w_\ell),
\end{equation}
where $l(w)$ denotes the length of $w$. Therefore we have $E[L_{TUNSTALL}(S)]=1.96$ for the example shown in Figure \ref{fig:tunstall example}.
\newline
Algorithm \ref{alg:tun} shows the Tunstall algorithm that finds the dicationary $\mathcal{D}$ for the source $S$ and a non-negative integer k such that $D=|S|+(|S|-1)k$, and $E[L_{TUNSTALL}(S)]$ from relation \ref{tunstall average} is maximized. For a tree t and set of strings {w}, t+$\{w\}$ means an extension of t by adding edges and nodes corresponding to the root-to-leaf paths given by strings $\{w\}$. The algorithm first starts by taking a tree with one internal node and each symbol as its children. Then for k iterations it finds the leaf node with the highest corresponding $p_{C}(w)$ and then expands that node by giving it $|S|$ children, each having an edge corresponding to a different symbol.
\newline
\newline
B. AIVF Coding
\begin{figure}[ht] 
    \centering
    \subfloat[The parse tree $t_0$]{
\begin{tikzpicture}[
node/.style={circle,draw,minimum width=7.3mm,inner sep=0}, level 1/.style={sibling distance=15mm},level distance=12mm, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)},baseline
]

\node [node]{\tiny $1.0$}
[child anchor=north]
child {node[node]{\tiny $0.6$}
child {node[node]{\tiny $0.36$} 
child {node[node]{\tiny $0.216$} 
child {node[node]{\tiny $0.1296$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}
}
  child {node[node]{\tiny $0.3$} 
  child {node[node]{\tiny $0.18$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
  edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}}
  child {node[node]{\tiny $0.1$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}};
\end{tikzpicture}}
\hspace{30pt}
%\hfill
%\renewcommand{\arraystretch}{1.3}
\subfloat[Dictionary Table of $\mathcal{D}(t_0)$]{
\begin{tabular}[t]{c|c|c}
$\ell$ & $w_{ \ell \in\mathcal{D}(t_0)}$  & $P_{C_{0}}(w_{ \ell})$                     \\ \hline
1 & $a_0$ & 0.24 \\ \hline
2 & $a_0 a_0$ & 0.144                     \\ \hline
3 & $a_0 a_0 a_0$ & 0.0864                     \\ \hline
4 & $a_0 a_0 a_0 a_0$  & 0.1296                      \\ \hline
5 & $a_1$  & 0.12                      \\ \hline
6 & $a_1 a_0$   & 0.18                       \\ \hline
7 & $a_2$   & 0.1                      
\end{tabular}}

    \subfloat[The parse tree $t_1$]{
\begin{tikzpicture}[
node/.style={circle,draw,minimum width=7.3mm,inner sep=0},noderight/.style={circle,draw,minimum width=7.3mm,inner sep=0, xshift={10mm}}, level 1/.style={sibling distance=15mm},level distance=12mm, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)},baseline
]
\node [node]{\tiny $1.0$}
[child anchor=north]
child {node[node]{\tiny $0.75$}
child {node[node]{\tiny $0.45$} 
child {node[node]{\tiny $0.27$} 
child {node[node]{\tiny $0.162$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
child {node[node]{\tiny $0.225$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}}
child {node[node]{\tiny $0.075$} edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}}
edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_1$}
}
  child {node[node]{\tiny $0.25$} 
  child {node[noderight]{\tiny $0.15$} edge from parent node[right,draw=none,yshift=0mm,xshift=0mm]{\small $a_0$}}
  edge from parent node[left,draw=none,yshift=0mm,xshift=0mm]{\small $a_2$}};
\end{tikzpicture}}
\hspace{30pt}
%\hfill
%\renewcommand{\arraystretch}{1.3}
\subfloat[Dictionary Table of $\mathcal{D}(t_1)$]{
\begin{tabular}[t]{c|c|c}
$\ell$ & $w_{ \ell \in\mathcal{D}(t_1)}$  & $P_{C_{1}}(w_{ \ell})$                     \\ \hline
1 & $a_1 a_0$ & 0.18 \\ \hline
2 & $a_1 a_0 a_0$ & 0.108                     \\ \hline
3 & $a_1 a_0 a_0 a_0$ & 0.162                     \\ \hline
4 & $a_1 a_1$  & 0.225                      \\ \hline
5 & $a_1 a_2$  & 0.075                      \\ \hline
6 & $a_2$   & 0.1                       \\ \hline
7 & $a_2 a_0$   & 0.15                      
\end{tabular}}
\caption{The optimal AIVF code for the source of $S=\{a_0,a_1,a_2\}$ and $p(a_0)=0.6$, $p(a_1)=0.3$, $p(a_2)=0.1$ and $D=7$.}
\label{fig:aivf example}
\end{figure}

The core difference between AIVF Coding and Tunstall coding is the usage of multiple dictionaries instead of one. The AIVF Code proposed by Yamamoto and Yokoo ~\cite{aivf-original} and extended by Dubé and Haddad ~\cite{dube-haddad} uses $|S|-1$ Dictionaries. Let $\{t_i | i\in\mathcal{I}_{|S|-1}\}$ denote the set of parse trees of these dictionaries and let $\mathcal{D}(t_i)$ denote the dictionary corresponding to the $t_i$ tree. We now explain the properties of the parse trees exactly as mentioned in ~\cite{AIVF-iterative}:
\begin{enumerate}
    \item[(p1)] If $v_j$ is the root of $t_i$, then $1\leq j\leq|S|-i$ and a different source symbol $a_u$, $u \in \{i,...,i+j-1\}$ is assigned to each of edges between the root and its children.
    \item[(p2)] If $v_j$ is a leaf, then $j=0$.
    \item[(p3)] If $v_j$ is an internal node, then $1 \leq j \leq |S|-2$ or $j=|S|$,
and a different source symbol $a_u$, $u\in\mathcal{I}_j$ is assigned to each of edges between node $v_j$ and its children.
\end{enumerate}

The dictionaries $\{\mathcal{D}(t_i)$ $|$ $i\in\mathcal{I}_{|S|-1}\}$ satisfy the exhaustive property which means that if $\mathcal{D}(t_i)$ is our current dictionary and our current source sequence is sufficiently large, then it is possible to match a prefix of the source sequence with a parseword from $\mathcal{D}(t_i)$. 
%This means that if we ignore the case where a few symbols might be left that cannot be parsed by the dictionary, we will n
\newline
In tree $t_i$, if a node $v_j$ is not the root and $0\leq j \leq |S|-2$, i.e. $v_j$ is not a complete internal node, then we assign a codeword to the node $v_j$. This means that we assign the codeword to the string $w\in S^{*}$ obtained by the path from the root to the node $v_j$, and we include $w$ to dictionary $\mathcal{D}(t_i)$. Let $\mathcal{D}_{i,j} \subset \mathcal{D}(t_i)$ be the set of parse strings obtained by the paths from the root to all $v_j$ for a fixed j in tree $t_i$.
If $v_j$ is the root of $t_i$ and $j<|S|-i$, we assign a codeword to the root, i.e. we assign the codeword to the empty string $\lambda$, and we add $\lambda$ to $\mathcal{D}_{i,i+j}$. Then, $\mathcal{D}(t_i)$ can be represented as $\mathcal{D}(t_i):= \prod_{j\in \mathcal{I}_{|S|-1}} \mathcal{D}_{i,j}$, $\mathcal{D}_{i,j} \cap \mathcal{D}_{i,j^{\prime}} = \emptyset$ for $j \neq j^{\prime}$.
Note that the root of $t_i$ has $|S|-i$ children at most, and hence the root can have $|S|$ children only in $t_0$.
\newline
A source sequence $s=s_1 s_2 ... s_n \in S^{n}$ is encoded by AIVF code with $\{\mathcal{D}(t_i)$ $|$ $i\in\mathcal{I}_{|S|-1}\}$ as follows.
\begin{enumerate}
    \item[(e1)] Use $t_0$ as the current tree for the first parsing of $s$.
    \item[(e2)] Obtain the longest prefix $w$ of $s$ in the current dictionary $\mathcal{D}(t_i)$ by tracing $s$ as long as possible from the root in the current tree $t_i$. Encode the obtained prefix $w$.
    \item[(e3)] If $w$ is included in $\mathcal{D}_{i,j} \subset \mathcal{D}(t_i)$, then use $t_j$ as the current tree for the next parsing. Remove $w$ from the prefix of $s$, and go to $(e2)$ if $s$ is not empty.
\end{enumerate}
Figure \ref{fig:aivf example} shows an example of AIVF code using the same parameters as our previous example. This AIVF code with $\{t_0,t_1\}$ encodes a source sequence ‘${a_1 a_0 a_0 a_0 a_1 a_0 a_0 a_2 a_0 a_2}$’ using the trees in the order of $t_0\rightarrow t_0\rightarrow t_1\rightarrow t_1\rightarrow t_0$ and deriving ‘$a_1 a_0$’, ‘$a_0 a_0$’, ‘$a_1 a_0 a_0$’, ‘$a_2 a_0$’, ‘$a_2$’ as the corresponding parsewords.
\newline Now we consider the probability $p_{W_i}(w)$ of phrase $w$ from the root to a node in tree $t_i$. We note from (p1)–(p3) and (e1)–(e3) that when $t_i$ is used to encode $s$ in (e2), the first symbol of $s$ is one of $a_u$, $u = i,...,|S|-1$. Therefore $p_{W_i}(w)$ can be calculated as follows.
\begin{equation} \label{eq:pwi}
     p_{W_i}(w)=
\begin{cases} 
      1 & $if $ w=\lambda, \\
      \frac{p_{W}(w)}{\sum_{u=i}^{|S|-1}p(a_u)} & $otherwise$
   \end{cases}
\end{equation}
Where $p_{W}(w)$ is given by \ref{eq:pw}.
\newline
We now consider the occurrence probability $p_{C_i}(w)$ for a phrase $w\in \mathcal{D}(t_i)$. The codewords are assigned to all leaves and all incomplete nodes in each $t_i$, and $w$ is used by the longest parse rule in the encoding. Then, $p_{C_i}(w)$ is given by
\begin{equation} \label{eq:pci}
    p_{C_i}(w)=p_{W_i}(w)-\sum_{\substack{a\in S s.t. \\ wa \preceq w^{\prime}\in \mathcal{D}(t_i)}} p_{W_i}(wa)
\end{equation}
where $wa\preceq w^{\prime} \in \mathcal{D}(t_i)$ means that $wa$ is a prefix of $w^{\prime}$
and $w^{\prime}\in \mathcal{D}(t_i)$.
\newline
In figure \ref{fig:aivf example} the value on each node indicates the $p_{W_i}(w)$ of the phrase $w$ derived from the path going from the root to the node, and you can see the value $p_{C_i}(w)$ for each $w\in \mathcal{D}(t_i)$ written in the tables.
\newline
The global average parse length of an AIVF code with $t=\{t_i | i \in \mathcal{I}_{|S|-1}\}$ for source S is given by
\begin{equation}
    E[L_{AIFV}(t,S)]:=\sum_{i\in \mathcal{I}_{|S|-1}}\pi(t_i)E[L_{t_i}(S)]
\end{equation}
where $\pi(t_i)$ indicates the stationary probability of $t_i$ in the encoding of a sufficiently long source sequence. By denoting $\boldsymbol{\pi}:=(\pi(t_0), \pi(t_1),..., \pi(t_{|S|-2}))$, we can calculate $\pi(t_i)$, $i \in \mathcal{I}_{|S|-1}$ from the following equations:
\begin{equation}
    \boldsymbol{\pi}Q=\boldsymbol{\pi}, \sum_{i\in \mathcal{I}_{|S|-1}}\pi(t_i)=1
\end{equation}
where $Q$ is a transition matrix of size $(|S|-1)\cdot(|S|-1)$, and the $(i, j)$-th element of $Q$ is given by a conditional probability $q(t_j|t_i)$ 
such that $t_j$ is used just after $t_i$ is used. If the prefix $w$ of a source sequence is included in $w \in D_{i,j}$ in the encoding by $t_i$, then $t_j$ is used for the next parsing. Hence, $q(t_j|t_i)$ is given by
\begin{equation}
    q(t_j|t_i)=\sum_{w\in D_{i,j}} p_{c_i}(w) \text{ for }  i,j \in \mathcal{I}_{|S|-1}.
\end{equation}
We therefore have $(E[L_{t_0}],E[L_{t_1}])=(1.8856,2.332)$ and $E[L_{AIFV}(t,S)]=2.10479$ for the example given in figure \ref{fig:aivf example}, which has a better coding rate than the corresponding Tunstall Code illustrated in Figure \ref{fig:tunstall example}.

==> WeaklyPolynomial.tex <==
In this section, we show that there exists a weakly polynomial time algorithm for constructing AIVF-m code of an alphabet $S=\{a_0,a_2,...,a_{m}\}$ such that the symbol $a_i$ is generated with probability $p(a_i)$. Assume we use $b$ bits to represent each floating point number. Thus, we can assume 
\[
    p(a_0) \geq p(a_1) \geq \dots \geq p(a_m) \geq 2^{-b}
\]

By the Proposition \ref{prop: main proposition for uniqueness}, there exists a unique multi-colored intersection point on $H$ which we know is the optimal solution. Also in Section \ref{sec: dp for aivf}, we introduced the Algorithm \ref{alg:dp} which calculates $\T(\x)$ for all $\x \in \R^{m-1}$ in polynomial time. By the Lemma 4.6 in ~\cite{golinaifv-m}, if we introduce a rectangle of a proper size such that it always contains the optimal solution, then, by ellipsoid algorithm, we can find the optimal solution in polynomial time based on $m$, $b$ and $D$ which is the size of the dictionary.

First, we prove a lemma that introduces a bounding box containing the highest point of $H$ if all probabilities and the cost function $\cost$ are bounded.

\begin{lemma} \label{lem: bounding lemma}
    Suppose $\States$ is a set of Markov chains defined in Section \ref{sec: intro} such that. $\cost$ is bounded by a positive real number $N$. Moreover assume $q_0(S_k) \geq 2^{-b}$ for all $1 \leq k \leq m-1$ and $S_k \in \States_k$. If $C \geq 2^b N$, then for all $i \in \langle m-1 \rangle$ the following statement holds:

    If $\x = [x_1,x_2,\dots,x_{m-1}]^T \in \R^{m-1}$ is such that $x_j \in [-C, C]$ for all $j \in \langle m-1 \rangle \setminus \{i\}$, we have:

    \begin{enumerate}
        \item If $x_i > C$ then $f_i \lp \x , S_i \rp < 0$
        \item If $x_i < -C$ then $f_i \lp \x , S_i \rp > N$
    \end{enumerate}
\end{lemma}

\begin{proof}
    We first show the first case. Note that
    \[
        f_i \lp \x , S_i \rp = \cost \lp S_i \rp  + \sum_{j=1}^{m-1}q_j \lp S_i \rp x_j - x_i
    \]
    Since for $j \in \langle m-1 \rangle \setminus \{i\}$ we have $x_j \in [-C, C]$, it is clear that the following inequality holds:
    
    \begin{equation} \label{eq: first ineq for lem}
        f_i \lp \x , S_i \rp \leq \cost \lp S_i \rp + \sum_{j \in \langle m-1 \rangle \setminus \{i\}} q_j \lp S_i \rp C - \lp 1 - q_i(S_i) \rp x_i
    \end{equation}
    
    We can rewrite the inequality (\ref{eq: first ineq for lem}) as follows:
    
    \[
        f_i \lp \x , S_i \rp \leq \cost \lp S_i \rp + \lp 1 - q_0(S_i) - q_i(S_i) \rp C - \lp 1 - q_i(S_i) \rp x_i
    \]
    We claim that
    \[
        N + \lp 1 - q_0(S_i) - q_i(S_i) \rp C - \lp 1 - q_i(S_i) \rp C \leq 0
    \]
    which is true if and only if
    \[
        q_0(S_i) C \geq N
    \]
    Note that $q_0(S_k) \geq 2^{-b}$ and $C \geq 2^b N$; therefore, the above inequality is true and the claim is proved. Moreover, one can easily conclude that the following holds:
    
    \[
        \cost \lp S_i \rp + \lp 1 - q_0(S_i) - q_i(S_i) \rp C - \lp 1 - q_i(S_i) \rp x_i < N + \lp 1 - q_0(S_i) - q_i(S_i) \rp C - \lp 1 - q_i(S_i) \rp C
    \]
    
    So, the first case of the lemma is proved.
    
    For the second part, by the similar conclusions as previous part we have
    \[
        f_i \lp \x , S_i \rp \geq \cost \lp S_i \rp -  \lp 1 - q_0(S_i) - q_i(S_i) \rp C - \lp 1 - q_i(S_i) \rp x_i
    \]
    Since $\cost \lp S_i \rp \geq 0$ we have
    \[
         f_i \lp \x , S_i \rp > -  \lp 1 - q_0(S_i) - q_i(S_i) \rp C + \lp 1 - q_i(S_i) \rp C = q_0(S_i)C \geq N
    \]
    and the lemma is proved.
\end{proof}

Here is the main theorem which introduces a bounding box for the optimal solution.

\begin{theorem}
    In the Lemma \ref{lem: bounding lemma}, the projection of the optimal multicolored point on $H$ lies inside $[-2^bN, 2^bN]^{m-1}$.
\end{theorem}

\begin{proof}
 By the Theorem \ref{prop: main proposition for uniqueness}, we know there exists a unique multicolored point on $H$. Moreover, by ~\cite[Theorem 3.1]{golinaifv-m} and the existence of the multicolored point on $H$, the minimum cost of any Markov chain in $\States$ is the height of the multicolored intersection point of their hyperplanes. Let $Q = [\x^*, h(\x^*)]^T$ and $S^* = (S^*_1, S^*_2, \ldots, S^*_{m-1})$ be the multicolored point on $H$ and the Markov chain associated to it. Assume $\x^* = [x_1,x_2,\ldots, x_{m-1}]^T$. Let $C = \max \{ |x_1| , \ldots, |x_{m-1}| \}$. If $\x^* \notin [-2^bN, 2^bN]^{m-1}$, then there exists index $i \in \langle m-1 \rangle$ s.t. 
 \[
    |x_i| \, \geq C > 2^bN
 \]
 We know $x_j \in [-C, C]$ for all $j \in \langle m-1 \rangle \setminus \{i\}$. Thus, by Lemma \ref{lem: bounding lemma}, we have two following cases:
 \begin{enumerate}
     \item $f_i \lp \x^*, S^*_i \rp < 0$
     \item $f_i \lp \x^*, S^*_i \rp > N$
 \end{enumerate}
 
 Since we know $h(\x^*) \geq 0$ and $N \geq cost(S^*)$ (because $Cost(S)$ is a convex combination of $\cost(S_i)$ for $i=0,\ldots,m-1$), non of the above can happen; contradiction. Thus the theorem is proved.
\end{proof}

Here is another statement that allows us to apply the Lemma \ref{lem: bounding lemma} to find a bounding box for the optimal solution of the AIVF-m Markov chain problem.

\begin{lemma} \label{lem: bounding cost}
    If $T = (T_0, T_1, \dots, T_{m-1})$ is an AIVF-m Markov chain with dictionary size at most $D$, then
    \[
        \cost (T_i) \leq D
    \]
    for all $0 \leq i \leq m-1$.
\end{lemma}

\begin{proof}
    
\end{proof}

Now by the Lemmas \ref{lem: bounding cost} and \ref{lem: bounding lemma} and the Lemma 4.6 in \cite{golinaifv-m}, we know there exists a weakly-polynomial time algorithm for constructing the optimal AIVF-m code.

For the $m=2$ case, a more implementable algorithm based on binary search exists which we will describe it in the sequel.

==> figure_1.tex <==

\begin{center}


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Right Triangle [id:dp5793948548228405] 
\draw   (348.69,59.47) -- (438,151.52) -- (348.69,151.52) -- cycle ;
%Shape: Triangle [id:dp6800804027061316] 
\draw   (268.83,80) -- (306.65,149.44) -- (231,149.44) -- cycle ;
%Shape: Free Drawing [id:dp45985273269334126] 
\draw  [line width=3] [line join = round][line cap = round] (268.83,81.39) .. controls (268.83,81.39) and (268.83,81.39) .. (268.83,81.39) ;
%Shape: Free Drawing [id:dp333344049270093] 
\draw  [line width=3] [line join = round][line cap = round] (348.69,59.47) .. controls (348.69,59.47) and (348.69,59.47) .. (348.69,59.47) ;
%Straight Lines [id:da9795118394244491] 
\draw    (268.83,80) -- (348.69,59.47) ;

% Text Node
\draw (297.55,47.18) node [anchor=north west][inner sep=0.75pt]    {$a_{i}$};
% Text Node
\draw (255.7,116.62) node [anchor=north west][inner sep=0.75pt]    {$s_{0}^{( l)}$};
% Text Node
\draw (359.88,118.93) node [anchor=north west][inner sep=0.75pt]    {$s_{i+1}^{( r)}$};
% Text Node
\draw (279.8,181.67) node [anchor=north west][inner sep=0.75pt]    {$Tie_{i}\left( s_{0}^{( l)} ,\ s_{i+1}^{( r)}\right)$};


\end{tikzpicture}


\end{center}


==> figure_2.tex <==

\begin{center}



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Triangle [id:dp529132917657509] 
\draw   (224.5,122.2) -- (267,185.2) -- (182,185.2) -- cycle ;
%Shape: Triangle [id:dp4493223588498969] 
\draw   (122.5,122.2) -- (165,185.2) -- (80,185.2) -- cycle ;
%Shape: Free Drawing [id:dp7479537809875545] 
\draw  [line width=3] [line join = round][line cap = round] (123,121.2) .. controls (123,121.2) and (123,121.2) .. (123,121.2) ;
%Shape: Free Drawing [id:dp9686820115883104] 
\draw  [line width=3] [line join = round][line cap = round] (225,122.2) .. controls (225,122.2) and (225,122.2) .. (225,122.2) ;
%Shape: Free Drawing [id:dp6283421271745495] 
\draw  [line width=3] [line join = round][line cap = round] (177,97.2) .. controls (177,97.2) and (177,97.2) .. (177,97.2) ;
%Straight Lines [id:da3611148556588055] 
\draw    (122.5,122.2) -- (177,97.2) ;
%Straight Lines [id:da19169633984154189] 
\draw    (177,97.2) -- (224.5,122.2) ;

% Text Node
\draw (108,153.4) node [anchor=north west][inner sep=0.75pt]    {$s_{0}^{( l)}$};
% Text Node
\draw (215,154.4) node [anchor=north west][inner sep=0.75pt]    {$s_{0}^{( r)}$};
% Text Node
\draw (115,89.4) node [anchor=north west][inner sep=0.75pt]    {$a_{\mid S \mid-2}$};
% Text Node
\draw (203,88.4) node [anchor=north west][inner sep=0.75pt]    {$a_{\mid S\mid-1}$};
% Text Node
\draw (128,201.4) node [anchor=north west][inner sep=0.75pt]    {$Tie_{\mid S \mid-2}\left( s_{0}^{( l)} ,\ s_{0}^{( r)}\right)$};


\end{tikzpicture}



\end{center}

